Training Multilingual Machine Translation by Alternately Freezing Language-Specific Encoders-Decoders

We propose a modular architecture of language-specific encoder-decoders that constitutes a multilingual machine translation system that can be incrementally extended to new languages without the need for retraining the existing system when adding new languages. Differently from previous works, we simultaneously train $N$ languages in all translation directions by alternately freezing encoder or decoder modules, which indirectly forces the system to train in a common intermediate representation for all languages. Experimental results from multilingual machine translation show that we can successfully train this modular architecture improving on the initial languages while falling slightly behind when adding new languages or doing zero-shot translation. Additional comparison of the quality of sentence representation in the task of natural language inference shows that the alternately freezing training is also beneficial in this direction.

==> sections/definitions.tex <==
Before defining the models implemented during this work, we may set some terminology to help understand the model. For all experiments, models are referred as encoder-decoder $e_i$, $d_i$ respectively for the \textit{i}th language in the system. For language independent scenarios, both encoder and decoder are considered independent modules that can be freely interchanged in order to produce all translation directions.

To refer to the freezing schedules employed in the language specific models, each language pair would be defined as a pair $f-n$,$n-f$,$n-n$ where the leftmost element points to the source language and the rightmost one to the target language and for each one it can either be $f$ for a frozen language or $n$ for a normally trained one.

==> sections/discussion.tex <==
%Recent literature focuses mainly on the use of shared encoder-decoder architectures for the task of Multilingual NMT. With this work we wanted to explore the possibilities of language specific encoder-decoders using state-of-the art techniques.

%Despite shared architectures still provide better results in most of the proposed experiments, this works shows that there is 

After analyzing the results on both tasks, we can further discuss the comparison among architectures.
%draw varius conclusions, especially on the situation of adding a new language. 

%When adding the new language (Russian), the language-specific encoder-decoders perform better in translation. However, in the cross-lingual natural language inference task, for this added language, the shared encoder-decoder outperforms the language-specific encoder-decoders with the greatest difference compared to the other XNLI cases (German, Spanish, French). This difference can be explained by the training schedule of each architecture. For Shared$^{RU}$, Russian shares its embedding table and parameters with English. 

The language-specific encoders-decoders just learn from the representation of the frozen modules without any common parameters. However, the frozen training schedule  introduces constraints on the  information that can flow between the different language-specific modules. Having to adapt to frozen components may force the model to learn representations that generalize better for downstream tasks. Further study would be needed for other tasks (e.g. question answering) and exploring other features present in the data to fully assert this hypothesis.

%While for translation, shared and frozen architectures provide comparable results (except for zero-shot), for natural language inference the shared model seems to be superior for not supervised languages (cross-lingual case), by a small amount. These results indicate that BLEU scores may not correlate well with generalization for downstream tasks, as other works have suggested before \cite{anonymous2020bertscore}.

%\todo[inline]{mikel: yo no enfocaria tanto en la aplicacion en downstream tasks. los resultados en xnli estan mas cerca de un random baseline (33\%) que del state-of-the-art (75-85\%), seguramente porque la estrategia de integracion no es optima, y no creo que se pueda sacar nada demasiado en claro de aqui. estos experimentos estan muy bien como analisis, pero la contribucion principal del paper esta en la parte del MT, y creo que conviene mantener esta perspectiva sin desviarse demasiado cuando la seccion viene a cerrar el paper}

 %Another detail to mention is the difference in performance in NLI between the supervised language, English, and the rest (XNLI). For both shared and language-specific, English shows a better performance and the frozen procedure shows the best results. When analyzing the results for SNLI English test set we can observe how this tendency is consistent.  This difference may be explained by how the frozen training schedule constraints the information that can flow between the different language-specific modules. Having to adapt to frozen components may force the model to learn representations that generalize better for downstream tasks. Further study would be required on other tasks, exploring other features present on the data to fully assert this hypothesis.



%Basic vs frozen. Differently from results in machine translation, here, we see no association between these results with the frozen directions trained. 


%Shared vs lang spec. Note that in the case of the added language (Russian), the language-specific encoders-decoders achieve lowest scores (10.8) compare to the shared procedure, which is precisely the task where language-specific improves over shared in machine translation. 

%\paragraph{Shared vs Shared$^{RU}$} When comparing the two shared configurations it is surprising that the model trained with less data provides the best results for this task, even though translation results where worse.

==> sections/implementation.tex <==



==> sections/related-work.tex <==
%\hl{TO DO}

Multilingual neural machine translation can refer to translating from one-to-many languages \cite{dong-etal-2015-multi}, from many-to-one \cite{zoph-knight-2016-multi} and many-to-many \cite{johnson2017google}. In this section, we briefly review the latter, which is the most general approach and also the one that we follow.

Within the many-to-many paradigm, existing approaches can be further divided into shared or language-specific encoder-decoders. The latter approaches vary from sharing parameters to no sharing at all. Among the common advantages of these approaches is that they allow for zero-shot translation; other properties are presented in what follows.% and summarized in Table \ref{tab:adv}. %\todo{mikel: cite en la caption para que salgan links}

\paragraph{Shared Encoder-Decoder.} \citet{johnson2017google} %\todo{mikel: cambio a citet para que linkee bien} 
feed a single encoder and decoder with multiple input and output languages. Given a set of languages, a shared architecture has a universal encoder $E_u$ and a universal decoder $D_u$ that are trained on all initial language pairs at once. The model shares parameters, vocabulary and tokenization among languages to ensure that no additional ambiguity is introduced in the representation. By sharing a single model across all languages, the system is able to represent all languages in a single space both semantically and lexically. This allows to translate between language pairs never seen during the training process just by sharing a common sentence representation, which is known as zero-shot translation.%, which translates in the ability to translate between directions that were never seen during training, zero-shot translation.
%As all languages are represented in the same token space, translation direction information has to be introduced to the model in order to decode the right target language. As proposed in previous works, we add a target language token to the source token representation to condition the decoding process. When adding new languages, the procedure is to retrain the entire system.
 This architecture provides a simple framework to develop multilingual systems because it does not require modifications of a standard neural machine translation model, and information is easily shared among the different languages through common parameters. Despite the model's advantages in transfer learning, the use of a shared vocabulary and embedding representation forces the model to employ a vocabulary that includes tokens from all the scripts used. Additionally, recent work \cite{DBLP:journals/corr/abs-1907-05019}, that imposes representational invariance across language, shows improvements in zero-shot translation but a decrease in performance in highly multilingual scenarios for high-resource languages. Therefore, increasing the number of languages varies the quality of the languages already in the system (generally enhancing low-resource pairs but being detrimental for high-resource pairs). Some other disadvantages are that the number of parameters related to vocabulary grow with the number of languages with different scripts and the entire system has to be retrained when adding new languages. 
%With this approach, authors show that zero-shot learning is possible. Authors show by means of visualizing similar sentences in different languages that there is some hint that these appear somehow close in the common representation. More recently, Arivazhagan et al (2019) \nocite{DBLP:journals/corr/abs-1903-07091} propose auxiliary losses on the neural machine translation encoder
%that impose representational invariance across languages, which is shown to improve zero-shot translation. Among the advantages, these architectures are efficient since only one encoder and one decoder is needed and low-resourced languages benefit directly from high-resourced languages. However, on the contrary, these architectures are detrimental for high-resourced languages, {\color{red} parameters related to vocabulary grows with the number of languages} and the entire system has to be retrained when adding new languages. 

\begin{comment}
\begin{table}[t]
    \fontsize{10pt}{10pt}\selectfont
    \centering
    \begin{tabular}{l|l|l|l}
         & Shared & \multicolumn{2}{c}{Lang-spec} \\\hline
         & &Partial & No \\ \hline
         Retraining for new lang & Yes & Yes & \bf No \\ \hline
         %Beneficial Low-Resources & Yes & Yes & Yes \\ \hline
         Translation quality varies & Yes & \bf Yes & \bf No \\ when adding lang  & & & \\ \hline
         Vocabulary Growth & Yes & \bf No & \bf No \\ \hline
%         Multi-way parallel corpus & \bf No & Yes &  \bf No \\ \hline
    \end{tabular}
    \caption{Comparison among approaches shared (Arivazhagan et al (2019)) and language-specific encoders-decoders (Lu et al., (2018), Escolano et al. (2019)).}
    \label{tab:adv}
\end{table}
\end{comment}

\paragraph{Language-specific Encoder-Decoders.} %These approaches vary from many encoders to one decoder (many-to-one) \cite{zoph:2016}, one encoder to many decoders (one-to-many) \cite{dong:2016} and, finally, one encoder to one decoder (one-to-one), which we are focusing on because they are closest to our approach. 
Approaches within this category may or may not share parameters at some point. %that partially share parameters have the commonality that they use language specific encoders and decoders and add a sharing step. 

\textit{Sharing parameters.} \citet{firat2016zero} proposed extending the bilingual recurrent neural machine translation architecture \cite{bahdanau2014neural} to the multilingual case \cite{vazquez-etal-2019-multilingual,lu2018neural} by designing a shared attention-based mechanism between the language-specific encoders and decoders to create a language independent representation.   These architectures provide the flexibility for each language to be trained with its own vocabulary, preventing problems related to the addition of several scripts in the same model, especially when some of them are underrepresented. However, as the language specific components rely on the shared modules, modifying those components to add a new language or add further data to the system would require retraining the whole system. 
\cite{DBLP:journals/corr/abs-1811-01137} proposes a model based on the addition of new languages to an already trained system by vocabulary adaptation and transfer learning. While limited, it requires some retraining to adapt the model to the new task; this results in the translation quality of existing languages varying when adding new ones.
%{\color{red}These architectures have the flexibility that each language can be trained with its own vocabulary, keeping the size, low}. However, because of sharing intermediate layers, {\color{red} the system (in most cases) has to be trained on a multi-way parallel corpus} and the entire system has to be retrained when adding new languages.

\textit{No sharing.}  The system proposed by \citet{escolano-etal-2019-bilingual} is trained on language-specific encoders and decoders based on joint training without parameter or vocabulary-sharing and on enforcing a compatible representation between the jointly trained languages. The advantage of the approach is that it does not require retraining to add new languages and increasing the number of languages does not vary the quality of the languages already in the system. However, the system has to be trained on a multiway\footnote{Multiway parallel corpus (between N languages) means a collection of texts aligned at the level of sentence between N languages} parallel corpus and the system does not scale well when there is a large number of languages in the initial system, since all encoders and decoders have to be trained simultaneously.



%{\color{red} CLARIFYy No veo por que el shared enc/dec y el ind enc/dec son distintos en cuanto al requerimiento de multi-way parallel corpus. Os referis a los recursos que se han usado en la literatura? O hay algo fundamental que no acabo de ver e impide usar un corpus multiligue parcial con los ind enc/dec?}

%limitacion de memoria, escalabilidad

